A copula-based method to build diffusion models with prescribed marginal and serial dependence

This paper investigates the probabilistic properties that determine the existence of space-time transformations between diffusion processes. We prove that two diffusions are related by a monotone space-time transformation if and only if they share the same serial dependence. The serial dependence of a diffusion process is studied by means of its copula density and the effect of monotone and non-monotone space-time transformations on the copula density is discussed. This provides us a methodology to build diffusion models by freely combining prescribed marginal behaviors and temporal dependence structures. Explicit expressions of copula densities are provided for tractable models. A possible application in neuroscience is sketched as a proof of concept.

==> bibl.tex <==
@book {ikeda,
    AUTHOR = {Ikeda, Nobuyuki and Watanabe, Shinzo},
     TITLE = {Stochastic differential equations and diffusion processes},
    SERIES = {North-Holland Mathematical Library},
    VOLUME = {24},
   EDITION = {Second},
 PUBLISHER = {North-Holland Publishing Co., Amsterdam; Kodansha, Ltd.,
              Tokyo},
      YEAR = {1989},
     PAGES = {xvi+555},
      ISBN = {0-444-87378-3},
   MRCLASS = {60H10 (58G32 60J60)},
  MRNUMBER = {1011252 (90m:60069)},
}




@article {nonnormalOU,
    AUTHOR = {Jensen, Jens Ledet and Pedersen, Jan},
     TITLE = {Ornstein-{U}hlenbeck type processes with non-normal
              distribution},
   JOURNAL = {J. Appl. Probab.},
  FJOURNAL = {Journal of Applied Probability},
    VOLUME = {36},
      YEAR = {1999},
    NUMBER = {2},
     PAGES = {389--402},
      ISSN = {0021-9002},
     CODEN = {JPRBAM},
   MRCLASS = {60J60 (60G10 62P05)},
  MRNUMBER = {1724832 (2000h:60076)},
}


@incollection{hyperbolicinfinance,
title = "Chapter 6 - Hyperbolic Processes in Finance ",
editor = "Rachev, Svetlozar T. ",
booktitle = "Handbook of Heavy Tailed Distributions in Finance ",
publisher = "North-Holland",
edition = "",
address = "Amsterdam",
year = "2003",
volume = "1",
pages = "211 - 248",
series = "Handbooks in Finance",
issn = "15684997",
doi = "http://dx.doi.org/10.1016/B978-044450896-6.50008-X",
url = "http://www.sciencedirect.com/science/article/pii/B978044450896650008X",
author = "Bo Martin Bibby and Michael S{\o}rensen",
}


@article {juliesorensenMM,
    AUTHOR = {Forman, Julie Lyng and S{\o}rensen, Michael},
     TITLE = {A transformation approach to modelling multi-modal diffusions},
   JOURNAL = {J. Statist. Plann. Inference},
  FJOURNAL = {Journal of Statistical Planning and Inference},
    VOLUME = {146},
      YEAR = {2014},
     PAGES = {56--69},
      ISSN = {0378-3758},
   MRCLASS = {60J60 (62M05)},
  MRNUMBER = {3132479},
MRREVIEWER = {Rosa Maria Mininni},
       DOI = {10.1016/j.jspi.2013.09.013},
       URL = {http://dx.doi.org/10.1016/j.jspi.2013.09.013},
}


@article {givencovariance,
    AUTHOR = {Bibby, Bo Martin and Skovgaard, Ib Michael and S{\o}rensen,
              Michael},
     TITLE = {Diffusion-type models with given marginal distribution and
              autocorrelation function},
   JOURNAL = {Bernoulli},
  FJOURNAL = {Bernoulli. Official Journal of the Bernoulli Society for
              Mathematical Statistics and Probability},
    VOLUME = {11},
      YEAR = {2005},
    NUMBER = {2},
     PAGES = {191--220},
      ISSN = {1350-7265},
   MRCLASS = {60J60 (60H10 60H30 62-07)},
  MRNUMBER = {2132002 (2005k:60249)},
       DOI = {10.3150/bj/1116340291},
       URL = {http://dx.doi.org/10.3150/bj/1116340291},
}


@article{
year={1996},
issn={0949-2984},
journal={Finance and Stochastics},
volume={1},
number={1},
doi={10.1007/s007800050015},
title={A hyperbolic diffusion model for stock prices},
url={http://dx.doi.org/10.1007/s007800050015},
publisher={Springer-Verlag},
keywords={Key words: Martingale estimating function; option pricing; quasi-likelihood; simulation; stochastic differential equation; volatility.; JEL classification: G12; Mathematics Subject Classification (1991): 62M05},
author={Bibby, Bo Martin and Sorensen, Michael},
pages={25-41},
language={English}
}

@article {mikoschcopulae,
    AUTHOR = {Mikosch, Thomas},
     TITLE = {Copulas: tales and facts},
   JOURNAL = {Extremes},
  FJOURNAL = {Extremes. Statistical Theory and Applications in Science,
              Engineering and Economics},
    VOLUME = {9},
      YEAR = {2006},
    NUMBER = {1},
     PAGES = {3--20},
      ISSN = {1386-1999},
   MRCLASS = {60E05 (60G70)},
  MRNUMBER = {2327842},
       DOI = {10.1007/s10687-006-0015-x},
       URL = {http://dx.doi.org/10.1007/s10687-006-0015-x},
}



@article {darsow,
    AUTHOR = {Darsow, William F. and Nguyen, Bao and Olsen, Elwood T.},
     TITLE = {Copulas and {M}arkov processes},
   JOURNAL = {Illinois J. Math.},
  FJOURNAL = {Illinois Journal of Mathematics},
    VOLUME = {36},
      YEAR = {1992},
    NUMBER = {4},
     PAGES = {600--642},
      ISSN = {0019-2082},
     CODEN = {IJMTAW},
   MRCLASS = {60J99 (46N30)},
  MRNUMBER = {1215798 (94h:60126)},
MRREVIEWER = {B. Schweizer},
       URL = {http://projecteuclid.org/euclid.ijm/1255987328},
}

@article {MR2668904,
    AUTHOR = {Lager{\aa}s, Andreas N.},
     TITLE = {Copulas for {M}arkovian dependence},
   JOURNAL = {Bernoulli},
  FJOURNAL = {Bernoulli. Official Journal of the Bernoulli Society for
              Mathematical Statistics and Probability},
    VOLUME = {16},
      YEAR = {2010},
    NUMBER = {2},
     PAGES = {331--342},
      ISSN = {1350-7265},
   MRCLASS = {60J25 (60J10 62H05)},
  MRNUMBER = {2668904 (2011i:60137)},
       DOI = {10.3150/09-BEJ214},
       URL = {http://dx.doi.org/10.3150/09-BEJ214},
}








@article {alzer,
    AUTHOR = {Alzer, Horst},
     TITLE = {On some inequalities for the gamma and psi functions},
   JOURNAL = {Math. Comp.},
  FJOURNAL = {Mathematics of Computation},
    VOLUME = {66},
      YEAR = {1997},
    NUMBER = {217},
     PAGES = {373--389},
      ISSN = {0025-5718},
       DOI = {10.1090/S0025-5718-97-00807-7},
       URL = {http://dx.doi.org/10.1090/S0025-5718-97-00807-7},
}



@article{griffith,
author={Griffith, M. and Courtney, T. and Peccoud, J. and Sanders, W.H.},
title={Dynamic partitioning for hybrid simulation of the bistable {HIV}-1 transactivation network},
journal={Bioinformatics},
year={2006},
volume={22},
number={22},
pages={2782-2789},
}



@article{salis2,
author={Salis, H. and Sotiropoulos, V. and Kaznessis, Y.N.},
title={Multiscale Hy3S: Hybrid stochastic simulation for supercomputers},
journal={BMC Bioinformatics},
year={2006},
volume={7},
page_count={21},
art_number={93},
}





@incollection{gshs,
year={2006},
isbn={978-3-540-33466-8},
booktitle={Stochastic Hybrid Systems},
volume={337},
series={Lecture Notes in Control and Information Science},
editor={Blom, HenkA.P. and Lygeros, John},
title={Toward a General Theory of Stochastic Hybrid Systems},
publisher={Springer Berlin Heidelberg},
author={Bujorianu, ManuelaL. and Lygeros, John},
pages={3-30},
language={English}
}



@inproceedings{pola2003stochastic,
  title={Stochastic hybrid models: An overview},
  author={Pola, G and Bujorianu, ML and Lygeros, J and Benedetto, MDD},
  booktitle={Proc. IFAC Conf. Anal. Design Hybrid Syst},
  pages={45--50},
  year={2003}
}



@article{caravagna,
Author = {Caravagna, Giulio and d'Onofrio, Alberto and Antoniotti, Marco. and
   Mauti, Giancarlo},
Title = {{Stochastic Hybrid Automata with delayed transitions to model biochemical
   systems with delays}},
Journal = {{INFORMATION AND COMPUTATION}},
Year = {{2014}},
Volume = {{236}},
Number = {{SI}},
Pages = {{19-34}},
DOI = {{10.1016/j.ic.2014.01.010}},
ISSN = {{0890-5401}}
}




@article{pdmp,
     jstor_articletype = {research-article},
     title = {Piecewise-Deterministic Markov Processes: A General Class of Non-Diffusion Stochastic Models},
     author = {Davis, M. H. A.},
     journal = {Journal of the Royal Statistical Society. Series B (Methodological)},
     jstor_issuetitle = {},
     volume = {46},
     number = {3},
     jstor_formatteddate = {1984},
     pages = {pp. 353-388},
     ISSN = {00359246},
     language = {English},
     year = {1984},
     publisher = {Wiley for the Royal Statistical Society},
     copyright = {Copyright © 1984 Royal Statistical Society},
    }




@incollection{lyg1,
year={2000},
isbn={978-3-540-67259-3},
booktitle={Hybrid Systems: Computation and Control},
volume={1790},
series={Lecture Notes in Computer Science},
editor={Lynch, Nancy and Krogh, BruceH.},
title={Towards a Theory of Stochastic Hybrid Systems},
publisher={Springer Berlin Heidelberg},
author={Hu, Jianghai and Lygeros, John and Sastry, Shankar},
pages={160-173},
language={English}
}

@book {karlin,
    AUTHOR = {Karlin, Samuel and Taylor, Howard M.},
     TITLE = {A second course in stochastic processes},
 PUBLISHER = {Academic Press, Inc. [Harcourt Brace Jovanovich, Publishers],
              New York-London},
      YEAR = {1981},
     PAGES = {xviii+542},
      ISBN = {0-12-398650-8},
   MRCLASS = {60-01 (60J60)},
  MRNUMBER = {611513 (82j:60003)},
MRREVIEWER = {D. A. Darling},
}



@article {feller1d,
    AUTHOR = {Feller, William},
     TITLE = {Diffusion processes in one dimension},
   JOURNAL = {Trans. Amer. Math. Soc.},
  FJOURNAL = {Transactions of the American Mathematical Society},
    VOLUME = {77},
      YEAR = {1954},
     PAGES = {1--31},
      ISSN = {0002-9947},
   MRCLASS = {60.0X},
  MRNUMBER = {0063607 (16,150d)},
MRREVIEWER = {R. S. Phillips},
}


@article {fellerParabolic,
    AUTHOR = {Feller, William},
     TITLE = {The parabolic differential equations and the associated
              semi-groups of transformations},
   JOURNAL = {Ann. of Math. (2)},
  FJOURNAL = {Annals of Mathematics. Second Series},
    VOLUME = {55},
      YEAR = {1952},
     PAGES = {468--519},
      ISSN = {0003-486X},
   MRCLASS = {36.0X},
  MRNUMBER = {0047886 (13,948a)},
MRREVIEWER = {K. Yosida},
}


@book{ErdiLente,
  title={Stochastic Chemical Kinetics},
  author={{\'E}rdi, P{\'e}ter and Lente, G{\'a}bor},
  isbn={978-1-4939-0386-3},
  series={Springer Series in Synergetics},
  year={2014},
  publisher={Springer}
}


@article{AAAHVW,
  author = {Angius, Alessio and Horv{\'a}th, Andr{\'a}s and Wolf, Verena},
  editor = {Priami, Corrado and Petre, Ion and {De Vink}, Erik},
  journal = {Transactions on Computational Systems Biology},
  number = {XIV},
  series = {Lecture Notes in Computer Science},
  title = {Quasi product form approximation for Markov models of reaction networks},
  volume = {7625},
  year = {2012}
}


@Article{MaWoDiHe10,
  author = 	 {M. Mateescu and V. Wolf and F. Didier and T. A. Henzinger },
  title = 	 {Fast adaptive uniformisation of the chemical master equation},
  journal = 	 {IET systems biology},
  year = 	 2010,
  volume =	 4,
  number =	 6,
  pages =	 {441--452}
}
@article{ZhWaCa10,
title = "A modified uniformization method for the solution of the chemical master equation",
journal = "Computers \& Mathematics with Applications",
volume = "59",
number = "1",
pages = "573 - 584",
year = "2010",
author = "J. Zhang and L. T. Watson and Y. Cao",
}

@article{CoCoCo11,
  author    = {Francesca Cordero and
               Andr{\'a}s Horv{\'a}th and
               Daniele Manini and
               Lucia Napione and
               Massimiliano De Pierro and
               Simona Pavan and
               Andrea Picco and
               Andrea Veglio and
               Matteo Sereno and
               Federico Bussolino and
               Gianfranco Balbo},
  title     = {Simplification of a complex signal transduction model using
               invariants and flow equivalent servers},
  journal   = {Theor. Comput. Sci.},
  volume    = {412},
  number    = {43},
  year      = {2011},
  pages     = {6036-6057},
  ee        = {http://dx.doi.org/10.1016/j.tcs.2011.06.013},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}

@Article{AnHo11b,
  author = 	 {A. Angius and A. Horv\'ath},
  title = 	 {Product Form Approximation of Transient Probabilities in Stochastic Reaction
Networks},
 journal = {Electronic Notes on Theoretical Computer Science},
  year =	 2011,
volume = {277},
  pages =	 {3-14}
}



@article{CiDeHiCa09,
  author = 	 {F. Ciocchetta and A. Degasperi and J. Hillston and M. Calder},
  title = 	 {Some Investigations Concerning the {CTMC} and the ODE 
                  Model Derived from Bio-PEPA. },
 journal = {Electron. Notes Theor. Comput. Sci.},
 volume = 229,
 issue = 1,
 year = 2009,
 pages = {145--163}
}
@Article{ZhWaCa09,
  author = 	 {J. Zhang and L. T. Watson and Y. Cao},
  title = 	 {Adaptive aggregation method for the Chemical Master Equation},
  journal = 	 {Int. J. of Computational Biology and Drug Design},
  year = 	 2009,
  volume =	 2,
  number =	 2,
  pages =	 {134--148}
}

@InProceedings{DaMiWo10,
  author = 	 {T. Dayar and L. Mikeev and V. Wolf},
  title = 	 {On the Numerical Analysis of Stochastic {L}otka-{V}olterra Models},
  booktitle =	 {Proc. of the Workshop on Computer Aspects of 
Numerical Algorithms (CANAÃ¯Â¿Â½10)},
  year =	 2010,
pages = {289--296}
}

@inproceedings{verena,
  title={Hybrid numerical solution of the chemical master equation},
  author={Henzinger, Thomas A and Mikeev, Linar and Mateescu, Maria and Wolf, Verena},
  booktitle={Proceedings of the 8th International Conference on Computational Methods in Systems Biology},
  pages={55--65},
  year={2010},
  organization={ACM}
}

@article{menz,
  title={Hybrid Stochastic--Deterministic Solution of the Chemical Master Equation},
  author={Menz, Stephan and Latorre, Juan C and Schütte, Christof and Huisinga, Wilhelm},
  journal={Multiscale Modeling \& Simulation},
  volume={10},
  number={4},
  pages={1232--1262},
  year={2012},
  publisher={SIAM}
}


@incollection{andersonKurtz,
  title={Continuous time Markov chain models for chemical reaction networks},
  author={Anderson, David F and Kurtz, Thomas G},
  booktitle={Design and Analysis of Biomolecular Circuits},
  pages={3--42},
  year={2011},
  publisher={Springer}
}

@article{2012,
  title={Hybrid Behaviour of Markov Population Models},
  author={Bortolussi, Luca},
  journal={CoRR CoRR abs/1211.1643},
  year={2012}
}
@INPROCEEDINGS{hybridLimit, 
author={Bortolussi, L.}, 
booktitle={Quantitative Evaluation of Systems (QEST), 2011 Eighth International Conference on}, 
title={Hybrid Limits of Continuous Time Markov Chains}, 
year={2011}, 
month={Sept}, 
pages={3-12}
}

@conference {luca2010,
	title = {Limit behavior of the hybrid approximation of Stochastic Process Algebras},
	booktitle = {17th International Conference on Analytical and Stochastic Modeling Techniques and Applications (ASMTA 2010)},
	year = {2010},
	month = {16, 2010},
	pages = {367{\textendash}381},
	publisher = {Springer-Verlag},
	organization = {Springer-Verlag},
	author = {Luca Bortolussi},
	editor = {K. Al-Begain and D. Fiems and W.J. Knottenbelt}
}



@incollection{bortolussi2013,
  title={Model checking markov population models by central limit approximation},
  author={Bortolussi, Luca and Lanciani, Roberta},
  booktitle={Quantitative Evaluation of Systems},
  pages={123--138},
  year={2013},
  publisher={Springer}
}




@article{intep,
  title={Switching and diffusion models for gene regulation networks},
  author={Intep, Somkid and Higham, Desmond J and Mao, Xuerong},
  journal={Multiscale Modeling \& Simulation},
  volume={8},
  number={1},
  pages={30--45},
  year={2009},
  publisher={SIAM}
}




@book {yin,
    AUTHOR = {Yin, G. George and Zhu, Chao},
     TITLE = {Hybrid switching diffusions},
    SERIES = {Stochastic Modelling and Applied Probability},
    VOLUME = {63},
      NOTE = {Properties and applications},
 PUBLISHER = {Springer, New York},
      YEAR = {2010},
     PAGES = {xviii+395},
      ISBN = {978-1-4419-1104-9},
   MRCLASS = {60J60 (60J25 60J75 62L20 93-02 93C30 93E15)},
  MRNUMBER = {2559912 (2010i:60226)},
MRREVIEWER = {{\L}. Stettner},
       DOI = {10.1007/978-1-4419-1105-6},
       URL = {http://dx.doi.org/10.1007/978-1-4419-1105-6},
}


@article{salis,
  title={Accurate hybrid stochastic simulation of a system of coupled chemical or biochemical reactions},
  author={Salis, Howard and Kaznessis, Yiannis},
  journal={The Journal of chemical physics},
  volume={122},
  number={5},
  pages={054103},
  year={2005},
  publisher={AIP Publishing}
}





@article{haseltine,
  title={Approximate simulation of coupled fast and slow reactions for stochastic chemical kinetics},
  author={Haseltine, Eric L and Rawlings, James B},
  journal={The Journal of chemical physics},
  volume={117},
  number={15},
  pages={6959--6969},
  year={2002},
  publisher={AIP Publishing}
}






@book{segel,
  title={Enzyme kinetics: behavior and analysis of rapid equilibrium and steady state enzyme systems},
  author={Segel, I.H.},
  isbn={9780471774259},
  lccn={lc74026546},
  series={Wiley classics library},
  url={http://books.google.it/books?id=6uFqAAAAMAAJ},
  year={1975},
  publisher={Wiley}
}



@misc{Rurl,
    howpublished = {\url{http://www.r-project.org/}},
    key = {R},
    title = {{{R} webpage}}
}



@article{Goutsias2005,
    author = {John Goutsias},
    doi = {10.1063/1.1889434},
    journal = {The Journal of Chemical Physics},
    number = {184102},
    title = {{Quasiequilibrium approximation of fast reaction kinetics in stochastic biochemical systems}},
    volume = {122},
    year = {2005}
}


@Book{YiZh10,
  author = 	 {G. George Yin and Chao Zhu},
  title = 	 {Hybrid Switching Diffusions: Properties and Applications},
  publisher = 	 {Springer},
  year = 	 2010}

@article{PSP:2044020,
author = {Cox,D. R.},
title = {The analysis of non-Markovian stochastic processes by the inclusion of supplementary variables},
journal = {Mathematical Proceedings of the Cambridge Philosophical Society},
volume = {51},
issue = {03},
month = {7},
year = {1955},
pages = {433--441}
}

@Article{HoKuNiTr98,
  author = 	 {Horton, G. and Kulkarni, V. G. and Nicol, D. M. and Trivedi, K. S.},
  title = 	 { Fluid stochastic Petri nets: Theory, application,
and solution techniques},
  journal = 	 {Eur. J. Op. Res.},
  year = 	 1998,
  volume = 	 105,
  number = 	 1,
  pages = 	 {184--201}}

@Article{GrSeHoBo01,
  author = 	 {M. Gribaudo and M. Sereno and A. Horv\'ath and A. Bobbio},
  title = 	 {Fluid Stochastic {P}etri Nets Augmented with
Flush-out Arcs: Modelling and Analysis},
  journal = 	 {Discrete Event Dynamic Systems: Theory and Applications},
  year = 	 2001,
  volume = 	 11,
  pages = 	 {97--117}}

@article{Gi01,
    author = {Gillespie, D. T.},
    journal = {J Chem Phys},
    pages = {1716--1733},
    title = {{Approximate accelerated stochastic simulation of chemically
reacting systems}},
    volume = {115},
year = {2001}
}

@article{RaPeCaGi03,
    author = {Rathinam, M. and Petzold, L. R. and Cao, Y. and Gillespie, D. T.},
    journal = {J Chem Phys},
    number = {24},
    pages = {12784--12794},
    title = {{Stiffness in stochastic chemically reacting systems: {T}he implicit tau-leaping method}},
    volume = {119},
    year = {2003}
}


@article{CaGiPe05,
    author = {Cao, Y. and Gillespie, D. T. and Petzold, L. R.},
    journal = {J Chem Phys},
    number = {1},
    title = {{The slow-scale stochastic simulation algorithm}},
    volume = {122},
    year = {2005}
}


@article{Gillespie_1977,
     author = {Gillespie, Daniel T.},
     journal = {J. Phys. Chem.},
      number = {25},
    pages = {2340--2361},
      title = {{Exact stochastic simulation of coupled chemical reactions}},
     volume = {81},
    year = {1977}
}

@Book{Wi06,
  author = 	 {Wilkinson, D.J},
  title = 	 {Stochastic Modelling for
Systems Biology},
  publisher = 	 {Chapman \& Hall},
  year = 	 2006}

@Article{TuScBu04,
  author = 	 {T.E. Turner and S. Schnell and K. Burrage},
  title = 	 {Stochastic approaches for modelling in vivo
reactions},
  journal = 	 {Comp. Bio. Chem.},
  year = 	 2004,
  volume = 	 28,
  pages = 	 {165â178}}

@article{srivastava,
  title={Stochastic vs. deterministic modeling of intracellular viral kinetics},
  author={Srivastava, R and You, L and Summers, J and Yin, J},
  journal={Journal of Theoretical Biology},
  volume={218},
  number={3},
  pages={309--321},
  year={2002},
  publisher={Elsevier}
}

@InProceedings{ATPN14,
  author = 	 {M. Beccuti and E. Bibbona and A. Horv\'ath and R. Sirovich and A. Angius and G. Balbo},
  title = 	 {Analysis of {P}etri Net models through Stochastic Differential Equation},
  booktitle = {Proc. of International Conference on Application and Theory of Petri Nets and other models of concurrency (ICATPN'14)},
  year = 	 2014,
  address = 	 {Tunis, Tunisia},
  month = 	 {June},
  note = 	 {\href{http://arxiv.org/abs/1404.0975}{arXiv:1404.0975}}}

@conference {Jane,
	title = {Don{\textquoteright}t Just Go with the Flow: Cautionary Tales of Fluid Flow Approximation},
	booktitle = {EPEW 2012, and UKPEW 2012},
	series = {Lecture Notes in Computer Science},
	volume = {7587},
	year = {2012},
	pages = {156{\textendash}171},
	publisher = {Springer},
	organization = {Springer},
	keywords = {fluid approximation, PEPA, Stochastic process algebras},
	author = {Alireza Pourranjbar and Jane Hillston and Luca Bortolussi},
	editor = {Mirco Tribastone and Stephen Gilmore}
}



@book{Peterson81,
 author = "J.L. Peterson",
 title = "{Petri Net Theory and the Modeling of Systems}",
 year = {1981},
 isbn = {0136619835},
 publisher = {Prentice Hall PTR},
 address = {Upper Saddle River, NJ, USA},
 }
 
 
 @inproceedings{RML1993,
   author    = {V. Reddy AND M. Mavrovouniotis AND M. Liebman},
   title     = {{Petri net representation in metabolic pathways}},
   booktitle = {Proc. Int. Conf. Intelligent Systems for Molecular Biology},
   year      = 1993,
   pages     = {328-336}
}
 
 @article{GossPecoud1998,
   author    = {P. Goss AND J. Pecoud},
   title     = {Quantitative modeling of stochastic systems in molecular biology by using stochastic {Petri} nets},
   journal = {Proc. Natl. Acad. Sci.},
   volume     = {95},
   number    = 12,
   year      = 1998,
   pages     = {6750--6755}
}


@article{Hof1994,
  author    = {R. Hofest{\"a}dt},
  title     = {A {Petri} Net Application of Metabolic Processes},
  journal   = {Journal of System Analysis, Modeling and Simulation},
  volume    = {16},
  year      = {1994},
  pages     = {113-122}
}


@incollection{match98-1,
   author    = {E. Teruel and G. Franceschinis and M Silva},
   title     = "{Untimed Petri Nets}",
   booktitle = {{Performance Models for Discrete Event Systems with
                Synchronisations: Formalisms and Analysis Techniques}},
   year      = 1998,
   publisher = {Editorial KRONOS},
   url = {http://webdiis.unizar.es/GISED/?q=news/matchbook},
   address   = {Zaragoza, Spain},
   editor    = {G. Balbo AND M. Silva},
   pages     = {27-75}
}


@book{Fish1978,
 author = {Fishman, G. S.},
 title = {Principles of Discrete Event Simulation},
 year = {1978},
 isbn = {0471043958},
 publisher = {John Wiley \& Sons, Inc.},
 address = {New York, NY, USA},
}

@article{molloy:spn,
 author = {M. K. Molloy},
 title = {Performance Analysis Using Stochastic Petri Nets},
 journal = {IEEE Transactions on  Computers},
 volume = {31},
 number = {9},
 year = {1982},
 issn = {0018-9340},
 pages = {913--917},
 doi = {http://dx.doi.org/10.1109/TC.1982.1676110},
 publisher = {IEEE Computer Society},
 address = {Los Alamitos, California, USA}
 }





@article{Baarir201121,
title = "Lumping partially symmetrical stochastic models",
journal = "Performance Evaluation",
volume = "68",
number = "1",
pages = "21 - 44",
year = "2011",
note = "",
issn = "0166-5316",
doi = "10.1016/j.peva.2010.09.002",
url = "http://www.sciencedirect.com/science/article/pii/S0166531610001239",
author = "S. Baarir and M. Beccuti and C. Dutheillet and G. Franceschinis and S. Haddad",
keywords = "Markov chains",
keywords = "Lumpability",
keywords = "Stochastic Petri nets",
keywords = "Symmetries"
}

@misc{Matlab-url,
  title = "{MATLAB} webpage",
  key = "MATLAB",
  howpublished = "\url{http://www.mathworks.com/}"
}

@inproceedings{LiuHY12,
  author    = {F. Liu and
               M. Heiner and
               M. Yang},
  title     = "{An efficient method for unfolding colored Petri nets}",
  booktitle = {Winter Simulation Conference},
  year      = "2012",
  Month     = {Dec.},
  address   = {Berlin, Germany},
  Publisher = {IEEE Computer Society},
  pages     = "1-12",
  ee        = {http://dl.acm.org/citation.cfm?id=2430157},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}

@article{boucherie:characterisation,
    author = {R. J. Boucherie},
    title = {A Characterisation of independence for competing {M}arkov chains with applications to stochastic {P}etri nets},
    journal = {IEEE Transactions on Software Engineering},
    volume = {20},
    number = {7},
    pages = {536--544},
    year = {1994},
    publisher = {IEEE Computer Society},
    address = {Los Alamitos, California, USA}
}


@article{coleman:product.form,
 author = {J. L. Coleman and W. Henderson and P. G. Taylor},
 title = {Product form  equilibrium distributions and a convolution algorithm for {S}tochastic {P}etri nets},
 journal = {Performance Evaluation},
 volume = {26},
 year = {1996},
 pages = {159--180},
 Publisher = {Elsevier}
}

@article{TrGiHi12,
   author              = {M. Tribastone and
                          S. Gilmore and
                          J. Hillston},
   title               = {Scalable Differential Analysis of Process Algebra Models.},
   Journal             = {IEEE Trans. Software Eng.},
   Volume              = {38},
   Number              = {1},
   year                = {2012},
   pages               = {205-219},
   publisher           = {IEEE Computer Society},
   address             = {Los Alamitos, California, USA},
   ee                  = {http://doi.ieeecomputersociety.org/10.1109/TSE.2010.82},
}





@book{KeSn60,
   author    = {J.G. Kemeny AND J.L. Snell},
   title     = {Finite {Markov} Chains},
   year      = 1960,
   publisher = {Van Nostrand},
   address   = {Princeton, NJ}
}

@incollection{Bal-01,
   author    = {G. Balbo},
   title     = "{Introduction to Stochastic Petri Nets}",
   booktitle = {{Formal Methods and Performance Analysis, LNCS Vol. 2090}},
   year      = 2001,
   month     = {May},
   publisher = {Springer-Verlag},
   address   = {Berlin, Germany},
   editor    = {E. Brinksma AND H. Hermanns AND J.-P. Katoen},
   pages     = {84-155}
}

@inproceedings{Beccuti12,
 author = {M. Beccuti and G. Franceschinis},
 title = {Efficient simulation of stochastic well-formed nets through symmetry exploitation},
 booktitle = {Proceedings of the Winter Simulation Conference},
 series = {WSC '12},
 year = {2012},
 month = {Dec.},
 location = {Berlin, Germany},
 pages = {296:1--296:13},
 articleno = {296},
 numpages = {13},
 acmid = {2430158},
 publisher = {IEEE Computer Society},
 address = {Los Alamitos, California, USA}
}

@article{GaetaTSE96,
  author    = {R. Gaeta},
  title     = "{Efficient Discrete-Event Simulation of Colored Petri Nets}",
  journal   = {IEEE Transactions on Software Engineering},
  volume    = {22},
  number    = {9},
  year      = {1996},
  pages     = {629-639},
  publisher = {IEEE Computer Society},
  address = {Los Alamitos, California, USA}
}



@article{IPSiRe03,
title = "{On fluidification of Petri Nets: from discrete to hybrid and continuous models}",
journal = "Annual Reviews in Control ",
volume = "28",
number = "2",
pages = "253 - 266",
year = "2004",
note = "",
issn = "1367-5788",
doi = "10.1016/j.arcontrol.2004.05.002",
url = "http://www.sciencedirect.com/science/article/pii/S1367578804000288",
author = "M. Silva and L. Recalde",
}
@article{Ciardo12,
  author = {Ciardo, G. and Zhao, Y. and Jin, X.},
  booktitle = {T. Petri Nets and Other Models of Concurrency},
  journal = {T. Petri Nets and Other Models of Concurrency},
  pages = {51-95},
  publisher = {Springer},
  series = {Lecture Notes in Computer Science},
  title = "{Ten Years of Saturation: A Petri Net Perspective.}",
  volume = 5,
  year = 2012
}


@INPROCEEDINGS{DaviesKK02,
    author = {I. Davies and W. J. Knottenbelt and P. S. Kritzinger},
    title = {Symbolic methods for the state space exploration of GSPN models},
    booktitle = {Proc. 12th International Conference on Modelling Techniques and Tools for Computer Performance Evaluation (TOOLS'02), volume 2324 of LNCS},
    year = {2002},
    month = {April},
    pages = {188--199},
    address   = {London, UK},
    publisher = {Springer}
}


@INPROCEEDINGS{Bu93,
  AUTHOR =       "P. Buchholz",
  TITLE =        "{Aggregation and reduction techniques for hierarchical {GCSPNS}}",
  BOOKTITLE =    "Proc. of 5th   International Workshop on Petri Nets and Performance Models",
  YEAR =         "1993",
  MONTH =        "oct.",
  pages =        "23-32",
  address =      "Toulouse, France",
  publisher =    "IEEE Computer Society"
}

@INPROCEEDINGS{Va91,
 TITLE = "{Stubborn Set of Colored Petri Nets}",
 AUTHOR ="A. Valmari",
 booktitle  =   {ICATPN 91},
 publisher  =   {IEEE Computer Society},
 month      =   {June},
 pages      =   {102-121},
 year       =   {1991},
 address    =   {Gjern, Denmark}
}



@INPROCEEDINGS{BaBrSe94,
  AUTHOR =       "G. Balbo AND S.C. Bruell AND M. Sereno",
  TITLE =        "{Arrival theorems for product-form stochastic Petri Nets}",
  BOOKTITLE =    "ACM  SIGMETRICS",
  YEAR =         "1994",
  pages =        "87-97",
  address =      "Nashville, Tennessee (USA)",
  MONTH= "May",
  Publisher = "ACM"
}

@article{Knottenbelt2000,
title = "{A probabilistic dynamic technique for the distributed generation of very large state spaces}",
journal = "Performance Evaluation ",
volume = "39",
number = "1â4",
pages = "127 - 148",
year = "2000",
author = "W.J. Knottenbelt and P.G. Harrison and M.A. Mestern and P.S. Kritzinger",
}


@article{Holzmann98,
 author = {Holzmann, G. J.},
 title = "{An Analysis of Bitstate Hashing}",
 journal = {Form. Methods Syst. Des.},
 issue_date = {Nov. 1998},
 volume = {13},
 number = {3},
 month = nov,
 year = {1998},
 issn = {0925-9856},
 pages = {289--307},
 numpages = {19},
 publisher = {Kluwer Academic Publishers},
 address = {Hingham, MA, USA},
}


@Article{HKN+03,
author={H. Hermanns and M. Kwiatkowska and G. Norman and D. Parker and M. Siegle},
title="{On the use of {MTBDD}s for Performability Analysis and Verification of Stochastic Systems}",
journal={Journal of Logic and Algebraic Programming: Special Issue on Probabilistic Techniques for the Design and Analysis of Systems},
year={2003},
volume={56},
number={1-2},
pages={23--67},
month={},
note={},
key={}
}

@InProceedings{Der07,
author={S. Derisavi},
title="{A Symbolic Algorithm for Optimal {Markov} Chain Lumping}",
booktitle={Proc. 13th International Conference on Tools and Algorithms for the Construction and Analysis of Systems (TACAS'07)},
year={2007},
editor={O. Grumberg and M. Huth},
pages={139-154},
organization={},
publisher={Springer},
series={LNCS},
volume={4424},
address={},
month={},
note={},
key={}
}


@INPROCEEDINGS{Kwia2002,
 author = {Kwiatkowska, M. Z. and Mehmood, R.},
 title = "{Out-of-Core Solution of Large Linear Systems of Equations Arising from Stochastic Modelling}",
 booktitle = {Proceedings of the Second Joint International Workshop on Process Algebra and Probabilistic Methods, Performance Modeling and Verification},
 series = {PAPM-PROBMIV '02},
 year = {2002},
 month = {July},
 isbn = {3-540-43913-7},
 pages = {135--151},
 numpages = {17},
 acmid = {668442},
 publisher = {Springer-Verlag},
 address = {London, UK, UK},
}

@INPROCEEDINGS{Boud01,
    author = {A. Bell Boudewijn and E. Bell and B. R. Haverkort},
    title = "{Serial And Parallel Out-Of-Core Solution of Linear Systems arising from Generalised Stochastic Petri Nets}",
    booktitle = {In Proc. High Performance Computing 2001},
    year = {2001},
    month = {Dec.},
    address = {Hyderabad, India},
    pages = {22--26},
    publisher = {Springer}
}

@INPROCEEDINGS{Deav97,
    author = {D. D. Deavours and W. H. Sanders},
    title = "{An efficient disk-based tool for solving very large Markov models}",
    booktitle = { Proc. 9th Int. Conf. on Modelling Techniques and Tools for Computer Performance Evaluation},
    year = {1997},
    month = {June},
    address = {Saint Malo, France},
    pages = {58--71},
    publisher = {Springer-Verlag}
}

@article {1450,
title = "{On fluidization of discrete event models: observation and control of continuous Petri nets}",
journal = {Discrete Event Dynamic Systems: Theory and Applications},
volume = {21},
year = {2011},
month = {Dic.},
pages = {497},
chapter = {427},
author = {M. Silva and J. Julvez and C. Mahulea and C.R. Vazquez}
}

@inproceedings {1284,
title = "{On the Importance of the Deadlock Trap Property for Monotonic Liveness}",
booktitle = {Int. Workshop on Biological Processes and Petri Nets (BioPPN), A satellite event of Petri Nets 2010},
year = {2010},
month = {June},
address = {Braga, Portugal},
isbn = {978-972-8692-53-7},
pages = {39--54},
url = {http://www-dssz.informatik.tu-cottbus.de/publications/BioPPN_2010/BioPPN_braga_2010_proceedings.pdf},
author = {M. Heiner and C. Mahulea and M. Silva}

}


@book{JensenBooks,
 author = {Jensen, K.},
 title = {Coloured Petri nets. Basic Concepts, Analysis Methods and Practical Use (vol.1,2,3)},
 year = {1997},
  publisher = {Springer Inc.},
 address = {New York, NY, USA},
}

@book{BOABCDF95,
author = { Ajmone Marsan, M. and  Balbo, G. and Conte, G. and  Donatelli, S. and Franceschinis, G. },
year = {1995},
publisher = {J. Wiley},
title = {{Modelling with Generalized Stochastic Petri Nets}},
address = {New York, NY, USA},
}


@INPROCEEDINGS{Tr10,
author={Tribastone, M.},
booktitle={Quantitative Evaluation of Systems (QEST), 2010 Seventh International Conference on the},
title={Scalable Differential Analysis of Large Process Algebra Models},
year={2010},
month={sept.},
volume={},
number={},
pages={307},
address={Williamsburg, Virginia, USA},
publisher={IEEE Computer Society}
}

@inproceedings{T&T12,
  author    = {M. Tschaikowski and
               M. Tribastone},
  title     = {Exact Fluid Lumpability for Markovian Process Algebra},
  booktitle={Proceedings of the 23rd International Conference on Concurrency Theory: CONCUR 2012},
  year      = {2012},
  month     = {sept.},
  address   = {Newcastle upon Tyne, UK},
  publisher = {Springer},
  pages     = {380-394},
  ee        = {http://dx.doi.org/10.1007/978-3-642-32940-1_27}

}

@article{T&T13,
author = "M. Tschaikowski and M. Tribastone",
title = "Tackling continuous state-space explosion in a Markovian process algebra ",
journal = "Theoretical Computer Science ",
volume = "",
number = "0",
pages = " - ",
year = "2013",
note = "",
issn = "0304-3975",
doi = "http://dx.doi.org/10.1016/j.tcs.2013.08.016",
url = "http://www.sciencedirect.com/science/article/pii/S0304397513006403"
}

@article{HayBra10,
author = "R. A. Hayden and J. T. Bradley",
title = "A fluid analysis framework for a Markovian process algebra ",
journal = "Theoretical Computer Science ",
volume = "411",
number = "22â24",
pages = "2260 - 2297",
year = "2010",
note = "",
issn = "0304-3975",
doi = "http://dx.doi.org/10.1016/j.tcs.2010.02.001"
}

 BibTeX | BibTeX (beta) | EndNote | ACM Ref

@book{Hillston96,
 author = {Hillston, J.},
 title = {A compositional approach to performance modelling},
 year = {1996},
 isbn = {0-521-57189-8},
 publisher = {Cambridge University Press},
 address = {New York, NY, USA},
}

@Article{SIR27,
  AUTHOR    = {Kermack, W.O. and McKendrick, A.G.},
  TITLE     = {A Contribution to the mathematical Theory of Epidemics},
  JOURNAL   = {Proceedings of the Royal Society of London. Series A},
  YEAR      = {1927},
  VOLUME    = {115},
  NUMBER    = {772},
  PAGES     = {700--721},
  MONTH     = {Aug}
}

@Article{CDFH93,
  AUTHOR    = {Chiola,G and Dutheillet, C. and Franceschinis, G. and Haddad, S.},
  TITLE     = {Stochastic well-formed coloured nets for symmetric  modelling applications},
  JOURNAL   = {IEEE Trans. on Computers},
  YEAR      = {1993},
  VOLUME    = {42},
  NUMBER    = {11},
  PAGES     = {1343--1360},
  MONTH     = {nov}
}

@book{St95,
        author = {Stewart, W. J. },
        citeulike-article-id = {2768413},
        posted-at = {2008-05-09 14:55:42},
        priority = {2},
        publisher = {Princeton University Press},
        title = {Introduction to the Numerical Solution of {M}arkov Chains.},
        year = {1995},
        address = {Princeton, New Jersey, USA}

}


@Article{Ku70,
  author =      {T. G. Kurtz},
  title =      {Solutions of Ordinary Differential Equations as
                  Limits of Pure Jump {M}arkov Processes},
  journal =      {Journal of Applied Probability},
  year =      1970,
  volume =     1,
  number =     7,
  pages =     {49--58}
}

@inproceedings{BeWi12,
 author = {Beccuti, M. and Franceschinis, G.},
 title = {Efficient simulation of stochastic well-formed nets through symmetry exploitation},
 booktitle = {Proceedings of the Winter Simulation Conference},
 series = {WSC '12},
 year = {2012},
 month = {Dec.},
 location = {Berlin, Germany},
 pages = {296:1--296:13},
 articleno = {296},
 numpages = {13},
 url = {http://dl.acm.org/citation.cfm?id=2429759.2430158},
 publisher = {IEEE Computer Society},
 address = {Los Alamitos, California, USA}
}


@inproceedings{BabarBDM10,
  author    = {J. Babar and
               M. Beccuti and
               S. Donatelli and
               A. S. Miner},
  title     = {GreatSPN Enhanced with Decision Diagram Data Structures},
  booktitle = {Proceedings of Applications and Theory of Petri Nets, 31st International
               Conference, PETRI NETS 2010, Braga, Portugal, June 21-25,},
  location  = {Braga, Portugal},
  year      = {2010},
  month     = {June},
  pages     = {308-317},
  publisher = {IEEE Computer Society},
  address   = {Los Alamitos, California, USA}

}


@incollection{Conte95,
year={1995},
booktitle={Application and Theory of Petri Nets 1995},
volume={935},
series={Lecture Notes in Computer Science},
editor={De Michelis, Giorgio and Diaz, Michel},
title="{Parallel state space exploration for GSPN models}",
publisher={Springer Berlin Heidelberg},
address = {Turin, Italy},
author={Caselli, S. and Conte, G. and Marenzoni, P.},
pages={181-200}
}



@INPROCEEDINGS{Allmaier97,
    author = {S. C. Allmaier and M. Kowarschik and G. Horton},
    title = "{State Space Construction and Steady-State Solution of GSPNs on a Shared-Memory Multiprocessor}",
    booktitle = {in Proc. IEEE Int. Workshop Petri Nets and Performance Models (PNPM '97},
    year = {1997},
    month = {June},
    address = {Saint Malo, France},
    pages = {112--121},
    publisher = {IEEE Computer Society}
}


@INPROCEEDINGS{Bobb08,
author={Bobbio, A. and Gribaudo, M. and Telek, M.},
booktitle="{Quantitative Evaluation of Systems, 2008. QEST '08. Fifth International Conference on}",
title={Analysis of Large Scale Interacting Systems by Mean Field Method},
year={2008},
month = {Sept.},
address = {Saint Malo, France},
pages={215-224},
publisher = {IEEE Computer Society}
}

@INPROCEEDINGS{ Brad08,
booktitle	= {SIPEW'08, SPEC International Performance Evaluation Workshop, Darmstadt, 27-28 June 2008},
title		= {{Extracting Response Times from Fluid Analysis of Performance Models}},
volume		= {5119},
series		= {Lecture Notes in Computer Science},
author		= {Bradley, J. T. and Hayden, R. and Knottenbelt, W. J. and Suto, T.},
pages		= {29--43},
month		= {June},
year		= {2008},
publisher   = {Springer},
address     = {Darmstad, Germany},
url		    = {http://pubs.doc.ic.ac.uk/responsetimes-fluidanalysis/}
}


@INPROCEEDINGS{Hillston05,
author={Hillston, J.},
booktitle={Quantitative Evaluation of Systems, 2005. Second International Conference on the},
title="{Fluid flow approximation of PEPA models}",
year={2005},
pages={33-42}
}



@article{SaMe89,
 author = {Sanders, W. H. and Meyer, J. F.},
 title = {Reduced base model construction methods for stochastic activity networks},
 journal = {IEEE J.Sel. A. Commun.},
 issue_date = {September 2006},
 volume = {9},
 number = {1},
 month = Sep,
 year = {2006},
 issn = {0733-8716},
 pages = {25--36},
 numpages = {12},
 acmid = {2313903},
 publisher = {IEEE Press},
 address = {Piscataway, NJ, USA},
} 



@Article{GiHiRi,
  author =       "S. Gilmore AND J. Hillston AND M. Ribaudo",
  title =        "{An efficient algorithm for aggregating {PEPA} models}",
  journal =      "Software Engineering, IEEE Transactions",
  volume =       "27",
  number =       "5",
  pages =        "449-464",
  month =        {May},
  year =         "2001",
   publisher = {IEEE Computer Society}
}



@incollection{kurtz1976limit,
  title={Limit theorems and diffusion approximations for density dependent Markov chains},
  author={Kurtz, Thomas G},
  booktitle={Stochastic Systems: Modeling, Identification and Optimization, I},
  pages={67--78},
  year={1976},
  publisher={Springer}
}

@article{kurtz1978strong,
  title={Strong approximation theorems for density dependent Markov chains},
  author={Kurtz, Thomas G},
  journal={Stochastic Processes and Their Applications},
  volume={6},
  number={3},
  pages={223--240},
  year={1978},
  publisher={Elsevier}
}


@book {bremaud1999,
    AUTHOR = {Br{\'e}maud, Pierre},
     TITLE = {Markov chains},
    SERIES = {Texts in Applied Mathematics},
    VOLUME = {31},
      NOTE = {Gibbs fields, Monte Carlo simulation, and queues},
 PUBLISHER = {Springer-Verlag},
   ADDRESS = {New York},
      YEAR = {1999},
     PAGES = {xviii+444},
      ISBN = {0-387-98509-3},
   MRCLASS = {60J10 (60J27 60K05)},
  MRNUMBER = {1689633 (2000k:60137)},
MRREVIEWER = {Richard F. Serfozo},
}

@book {klebaner,
    AUTHOR = {Klebaner, Fima C.},
     TITLE = {Introduction to stochastic calculus with applications},
   EDITION = {Third},
 PUBLISHER = {Imperial College Press},
   ADDRESS = {London},
      YEAR = {2012},
     PAGES = {xiv+438},
      ISBN = {978-1-84816-832-9; 1-84816-832-2},
   MRCLASS = {60-01 (60H05 60H30 60J65 60J70 60J75 60J85)},
  MRNUMBER = {2933773},
}

@article{gillespie,
  title={The chemical Langevin equation},
  author={Gillespie, Daniel T},
  journal={J. Chem. Phys.},
  volume={113},
  pages={297},
  year={2000}
}

@article{pahle,
  title={Biochemical simulations: stochastic, approximate stochastic and hybrid approaches},
  author={J. Pahle},
  journal={Briefings in Bioinformatics},
  volume={10(1)},
  pages={53-64},
  year={2009}
}

@book {cont04,
    AUTHOR = {Cont, Rama and Tankov, Peter},
     TITLE = {Financial modelling with jump processes},
    SERIES = {Chapman \& Hall/CRC Financial Mathematics Series},
 PUBLISHER = {Chapman \& Hall/CRC, Boca Raton, FL},
      YEAR = {2004},
     PAGES = {xvi+535},
      ISBN = {1-5848-8413-4},
   MRCLASS = {91-02 (60J75 91B28 91B84)},
  MRNUMBER = {2042661 (2004m:91004)},
}


@book{rogers,
  title={Diffusions, Markov Processes, and Martingales: Volume 2, It$\bar{\mbox{o}}$ calculus.},
  author={Rogers, L Chris G and Williams, David},
  year={2000},
  publisher={Cambridge university press}
}



@book {discreteUnivariate,
    AUTHOR = {Johnson, Norman L. and Kemp, Adrienne W. and Kotz, Samuel},
     TITLE = {Univariate discrete distributions},
    SERIES = {Wiley Series in Probability and Statistics},
   EDITION = {Third},
 PUBLISHER = {Wiley-Interscience [John Wiley \& Sons], Hoboken, NJ},
      YEAR = {2005},
     PAGES = {xx+646},
      ISBN = {978-0-471-27246-5; 0-471-27246-9},
}




